Coordination-free Decentralised Federated Learning on Complex Networks: Overcoming Heterogeneity

Federated Learning (FL) is a well-known framework for successfully performing a learning task in an edge computing scenario where the devices involved have limited resources and incomplete data representation. The basic assumption of FL is that the devices communicate directly or indirectly with a parameter server that centrally coordinates the whole process, overcoming several challenges associated with it. However, in highly pervasive edge scenarios, the presence of a central controller that oversees the process cannot always be guaranteed, and the interactions (i.e., the connectivity graph) between devices might not be predetermined, resulting in a complex network structure. Moreover, the heterogeneity of data and devices further complicates the learning process. This poses new challenges from a learning standpoint that we address by proposing a communication-efficient Decentralised Federated Learning (DFL) algorithm able to cope with them. Our solution allows devices communicating only with their direct neighbours to train an accurate model, overcoming the heterogeneity induced by data and different training histories. Our results show that the resulting local models generalise better than those trained with competing approaches, and do so in a more communication-efficient way.

==> macros.tex <==
\def\*#1{\mathbf{#1}}

==> old/tnnls_body-old.tex <==
[Transactions on Neural Networks and Learning Systems, 10 pages w/o overlength charge, 200\$ per extra page]

\section{Introduction}
\label{sec:intro}
\IEEEPARstart{W}{e} are currently observing a significant shift within the realm of AI, as it moves away from the conventional centralized systems and embraces a decentralized approach. This paradigm shift is primarily driven by the changing attitudes of data generators situated at the network's edge. They have become increasingly hesitant to share their private data with third parties, even when promised potential benefits from centralized AI services.
%
To address these concerns, decentralized AI systems, such as Federated Learning (FL), have emerged as promising solutions. FL introduces innovative methodologies to tackle the challenges at hand. It involves keeping the data securely stored on edge devices, empowering them with a central role in the knowledge extraction process. Rather than sharing their raw data, these devices collaborate by sharing only the parameters obtained from their locally trained models. By aggregating these parameters, an enhanced global model is created, which undergoes further refinement through iterative collaboration rounds. This approach ensures privacy and enables data generators to actively participate in the AI training process without compromising their sensitive information. 

The standard FL framework assumes a centralized structure where a parameter server (PS) oversees the entire process and coordinates the operations of multiple clients. The challenges connected to FL are many and all related to the highly pervasive and heterogeneous environment where the client devices operate. Specifically, the local datasets held by devices might be non-iid, the devices might have different capabilities (e.g., computation, memory, battery) and  the connectivity might be intermittent, possibly preventing their participation to the distributed training\cite{}. All these challenges can be addressed or mitigated exploiting the central control of the PS. Specifically, the PS can synchronize the training by sharing the same model to the clients, it can select which clients' updates to include in the global model\cite{}, it can mitigate the data heterogeneity during the aggregation phase \cite{}, and more in general can control the overall progress of the distributed training. However, having a central controller can pose issues such as being a single point of failure, creating bottlenecks when dealing with millions of devices, and hindering direct collaborations between users. Moreover, having a central controller is not always feasible, i.e., in IoE scenarios, devices are expected to operate without a server because they are sometimes connected via multi-hop networks, through which devices can only communicate with adjacent ones\cite{}. 

In light of these considerations, in this paper we target a system where the central controller is absent. Precisely, we focus on a highly pervasive environment where a multitude of devices (e.g. personal mobile devices, IoT devices, etc) generate data and need an effective mechanism to collaboratively train a local model without any central coordination. We assume that the devices communicate between each others through a communication graph whose topology cannot be controlled or designed beforehand, as it would happen in a realistic edge environment. 

In these settings, since the standard FL methodologies based on centralization are not applicable anymore, we resort to Decentralised Federated Learning (DFL).  Briefly DFL is a generalization of Federated Learning where the devices are connected in a generic graph, and they typically collaborate only with their neighboring devices. 
%
% Decentralized Federated Learning (DFL) emerges to the centralized approach. In DFL, devices are connected in a generic graph, and they typically collaborate only with their neighboring devices. 
%
While the absence of a central controller in DFL resolves the single point of failure problem, it introduces new aspects that require investigation. For example, we argue that the information locality, lack of central orchestration, and the network topology may significantly impact the learning process dynamics, specifically how quickly and effectively knowledge embedded in the local models spreads over the network.
%
% Specifically, previous work~\cite{savazzi_federated_2020} has assumed that the network topology can be controlled and optimized by the network operator to enhance the efficiency and scalability of the learning process. However, we contend that true decentralization can only be achieved by allowing user devices to organize themselves spontaneously. In this case, the network topology cannot be controlled by the operator. Moreover, the connections between nodes in the graph may represent trust relationships or willingness to cooperate, with weighted edges indicating the strength of trust or cooperation. This approach grants users the freedom to cooperate with whomever they choose, while the operator has no control over the patterns of cooperation. Although this poses a challenge from a learning perspective, it fully harnesses the human-centric and impromptu potential of fully decentralized learning systems. 

Topology is not the only aspect that cannot be controlled in a decentralised edge scenario, data distribution and model heterogeneity are additional dimensions to consider. The former is a well known challenge due to the fact that, given a specific domain, the data collected by the edge devices might be unevenly represented across them, leading to a possible under-representation of data on some of the devices and to an over-representation to some others, creating unbalance in the data distribution between devices. The latter, instead, is less considered in the literature and it refers to a peculiar condition for a decentralised and uncoordinated scenario. Specifically, let us consider a massive number of devices spontaneously interconnected between each others, all committed to collaborate to train a common model (i.e., same topology) using their local data. It would be unlikely to assume that, at given point in time, all the devices across the network can agree spontaneously on a common initialisation, before starting the collaboration. 
% Specifically, if we consider a system with no central coordination it is not reasonable to assume the existence of a unique global model to train on the clients' data as in the standard Federated Learning framework. Even in presence of clients holding data belonging to the same ``application domain'' (e.g. images to classify, object to recognize, anomalies to identify, etc.), for which they might know which kind of model architecture to use (e.g. a LeNet, a VGG, etc.), 
Conversely, due the locality principle, it would be more realistic to consider that each of them has a model with a different initialisation or training status. Generalising, this represents a situation where the devices followed different training and collaboration histories before starting the collaboration, leading to a initial condition, from the decentralised learning standpoint, where their models are topologically far from each other. 

Under these assumptions, the research question we tackle in this paper targets all the three aspects mentioned so far: How to perform an \emph{efficient} decentralised federated learning task in a scenario where (i) there is \emph{no central coordination}, (ii) the interaction between nodes is constrained by a \emph{non-trivial topology}, (iii) \emph{data} is distributed heterogeneously across nodes, and (iv) \emph{clients' models} are not homogeneously initialised? 

% talk about local training and aggregation. Motivate and  highlight the idea behind both. 
% for virtual teacher: the usual approahcis to use KD on a common dataset. we do not want to share any data and we assume that all the models are weak learners. Therefore we remove the dependence from a real teacher by we rely on a so called virtual teacher. Following the ideas in \cite{} we substitute the output of a real teacher with a a hand crafted softlabelling and we train the local model through the KD Loss. 
% for the aggregation part we propose to overcome the drawbacks of FedAvg induced the model heterogeneity by proposing an aggregation function that takes into account the regulates the local model update proportinally to the difference between the local model and the average 
% sketch the main results. 


The main take-home messages are the following:
\begin{itemize}
    \item add take home messages
\end{itemize}

[When explaining the structure of the paper, put a forward pointer explaining why we present our contribution very later (sec. IV)]
The reminder of the paper is the following:  \autoref{sec:relwork} reviews the literature,  in \autoref{sec:problem_description} we define the problem and we discuss the approaches that represent the baselines of this work. \autoref{sec:contribution} we describe our contribution and in \autoref{sec:settings} and \autoref{sec:results} we present the experimental settings and discuss the performance evaluation, respectively. Finally in \autoref{sec:conclusion} we draw some conclusions. 
 
\section{Related work}
\label{sec:relwork}

Extensive research has been conducted on decentralized learning. Initial studies focused on computing the average of decentralized data, which is physically distributed across devices connected through a network topology resembling a graph. This scenario was particularly relevant for averaging data from sensor networks \cite{boyd_gossip_2005,aysal_broadcast_2009}. Subsequent investigations delved into Decentralized Gradient Descent (DGD) \cite{Nedic:2017aa, Yuan:2016aa} and examined its convergence properties under convexity assumptions. In their work \cite{zeng_nonconvex_2018}, the authors demonstrated that convergence does not strictly require convexity, opening the door for applying DGD to non-convex optimization problems. Apart from DGD, decentralized settings also attracted attention for Stochastic Gradient Descent (SGD). In their publication \cite{sirb_consensus_2016}, the authors proposed a decentralized SGD algorithm and provided guarantees for its convergence. Furthermore, the work in \cite{lian_can_2017} analyses the communication efficiency of DSGD, considering that the updates' exchange between nodes is synchronous. Their results show that decentralised SGD can be more efficient than centralised SGD, especially when the communication bandwidth is limited. The asynchronous version of DSGD is analysed in \cite{Lian2017}. 

Additionally, the research explored Decentralized Federated Learning, which extends the typical framework of Federated Learning by removing the need for a central parameter server that oversees and coordinates the learning process. This new area has gained significant interest as it combines the privacy advantages of Federated Learning with the potential of decentralized and uncoordinated optimization and learning. Research in this domain considers various factors such as data heterogeneity, non-convex optimization, and the absence of a central server. In their work \cite{Roy2019}, the authors defined a decentralized Federated Learning framework for a medical application involving multiple hospitals collaborating to train a Neural Network model on local and private data. Another approach, proposed in \cite{Lalitha2019,lalitha_fully_nodate}, adopts a Bayesian-like strategy where the aggregation phase minimizes the Kullback-Leibler divergence between the local model and the received models from peers. While most approaches assume a single local update before sharing parameters or gradients with peers, this assumption is relaxed in \cite{savazzi_federated_2020} and \cite{sun_decentralized_2022}. \cite{savazzi_federated_2020} presents a federated consensus algorithm, extending Federated Avg to decentralized settings, focusing on industrial and IoT applications. \cite{sun_decentralized_2022} propose Federated Decentralized Average based on SGD, incorporating a momentum term to counteract potential drift introduced by multiple updates and a quantization scheme to enhance communication efficiency. A comprehensive review of decentralised learning algorithms can be found in \cite{bellavista2021}.

While the works in the literature do consider data-related heterogeneity, i.e., non-IID data across devices, all of them assume to have a homogeneous system from the model point of view, i.e., all the models share the same initialization. To the best of our knowledge, for the first time, we relax this assumption by considering a fully decentralised learning system where not only data is spread in a non-IID fashion in the system but also the models are \emph{initialised heterogeneously}. We propose a solution for dealing with the detrimental effects that such heterogeneity introduces in the learning process.  

% TODO to be extended

% Decentralised learning has been extensively investigated. Initial papers investigated the problem of computing the average over a set of decentralised data physically located on a set of devices connected through a graph-like network topology (e.g., the enabling scenario was related to averaging data from sensor networks) \cite{boyd_gossip_2005,aysal_broadcast_2009}. Further studies investigated Decentralised Gradient Descent (DGD) \cite{Nedic:2017aa, Yuan:2016aa}, analysing its convergence properties under convexity assumptions. In \cite{zeng_nonconvex_2018}, the authors prove that convexity is not a strict requirement for convergence, paving the way for using DGD to address problems of non-convex optimisation. Beyond DGD, also SGD received attention in decentralised settings. In  \cite{sirb_consensus_2016}, the authors proposed a decentralised SGD algorithm and provided convergence guarantees.
% Furthermore, the paper in \cite{lian_can_2017} analyses the communication efficiency of DSGD, considering that the updates' exchange between nodes is synchronous. Their results show that decentralised SGD can be more efficient than centralised SGD, especially when the communication bandwidth is limited. The asynchronous version of DSGD is analysed in \cite{Lian2017}. 

% A different research line investigates Decentralised Federated Learning, which extends the typical settings of Federated Learning, e.g., data heterogeneity and non-convex optimisation, to mention a few. , by removing the existence of a central parameter server, which typically oversees and coordinates the whole learning process. This is a relatively new topic which is gaining attention from the community since it fuses the privacy-related advantages of Federated Learning with the potentialities of decentralised and uncoordinated optimisation and learning. 
%  % that the information shared with the peers is communicated right after one local update. Others relax this assumption, considering multiple local updates to the local model before sharing the local parameters or the local gradients with the peers.
% In \cite{Roy2019}, the authors define a decentralised Federated Learning framework for a medical application where a number of hospitals collaborate to train a Neural Network model on local and private data. In \cite{Lalitha2019,lalitha_fully_nodate} propose a Bayesian-like approach where the aggregation phase is done by minimising the Kullbac-Leibler divergence between the local model and the ones received from the peers. All these approaches are still considering that the nodes perform just one local update before sharing the parameters (or gradients) with the peers in the network. This aspect is relaxed in \cite{savazzi_federated_2020} and \cite{sun_decentralized_2022}. In \cite{savazzi_federated_2020}, the authors propose a federated consensus algorithm extending Federated Avg in decentralised settings, mainly considering industrial and IoT applications. The paper \cite{sun_decentralized_2022} proposes a Federated Decentralised Average based on SGD where the authors include a momentum term to counterbalance the possible drift introduced by the multiple updates and a quantization scheme to make the solution communication efficient. 
%%% DECENTRALIZATION but not really
% short notes on papers we have recently considered as benchmarks. to be properly integrated with the related work
% \cite{sun_decentralized_2023}: they focus on introducing a heavy ball momentum into FedAVg (the version in~\cite{mcmahan_communication-efficient_2017} had no momentum). In addition, they consider pairwise communications among nodes (no central server). Their DFedAvgM is basically equivalent to the DecAvg strategy we discuss in Section~\ref{sec:contribution}. Note also that this paper does not assume any underlying network topology. They work under the assumption that any node can communicate with any other node, but there is an overlay layer that filters such communications in a way that the number of neighbors is controlled by the system designer. 

% \cite{li_decentralized_2022}

%==========================================================================
\section{Problem description}
\label{sec:problem_description}

\subsection{Preliminaries}
\label{sec:preliminaries}
 We consider a graph $\mathcal{G}(\mathcal{V},\mathcal{E})$ where $\mathcal{V}$ denotes the set of nodes and $\mathcal{E}$ the set of edges. Without loss of generality, we assume that the nodes are edge devices and that the existence of an edge between a pair of nodes means that the two nodes are willing to collaborate with each other in a supervised learning task, and thus can exchange related information such as models' parameters. Without loss of generality, we focus on a multi-class classification problem. In our system, the graph is a generic representation of a communication topology between devices thus, we assume that the edges (i.e., the links between nodes) can be weighted, i.e., we associate a scalar value $\omega_{ij} \in \mathbb{R}$ to the edge connecting nodes $i,j \in \mathcal{V}$. In this way we enable different interpretations of the graph, which can represent, e.g., a social network where the links represent the level of trust or social intimacy between two nodes. 

Each node $i\in \mathcal{V}$ holds a local dataset $D_i$ a set of samples $\{\*x_k,y_k\}_{k=1}^{|D_i|}$. 

 Each $\*x_k\in\mathcal{X}_i\subseteq\mathcal{X}$, $\mathcal{X}_i$ denotes the local input space and $\mathcal{X}$ the global input space satisfying $\bigcup_{i=1}^{|\mathcal{V}|}\mathcal{X}_i \subseteq \mathcal{X}$. The $k$-th label $y_k$ for node $i$ is given by $y_k = h(\*x_k;\*w^*)+\eta_i$, where $h(\cdot)$ is a parametric function defined as $h(\cdot;\*w^*):\mathcal{X} \rightarrow \mathcal{Y}$, $\*w^*$ denotes the fixed global ``true parameters'' belonging to the set $W\subseteq\mathcal{W}$ (the parameters space) and $\eta_i$ denotes independent additive noise at node $i$. The global true parameters $\*w^*$ are unknown to the nodes/devices. Furthermore, we assume that the local training datasets are generated locally on nodes and that there is no data overlapping between them. Moreover, we assume that the distribution of samples per class is \emph{non-IID} across nodes, and that the total amount of samples is in general different across nodes. Following the taxonomy in~\cite{kairouz_advances_2021}, we focus on quantity and label distribution skew. 
 
 


%================================================================================
\subsection{Non-decentralized baseline strategies}
\label{sec:baselines_nondec}

In the following, we describe the standard baselines for non-decentralized learning. While they cannot work in a fully decentralized domain, they still provide a reference point for comparison to understand the accuracy that could be achieved under a different, more controllable, distributed configuration. For each of them, we briefly summarise the corresponding communication overhead. The communication overhead is an important property to consider in fully decentralized settings, as intense network usage can rapidly drain mobile devices' batteries and, depending on the network in use (cellular, WiFi, etc.), consume the mobile data monthly cap.

\noindent {\bf{Central learning:}} All the data are on a central server and the reference model is trained on it. There is a single model in the network, which we denote with $h(\cdot; \*w_g)$.

\noindent{}\emph{Communication overhead}: nodes send, once, all their data items to the central server.

\noindent {\bf{Federated learning - FedAvg~\cite{mcmahan_communication-efficient_2017}:}} FedAvg is the most popular instance of the Federated Learning paradigm. As in all federated learning scenarios, data are scattered across client devices (which would correspond to the nodes in $\mathcal{V}$, which communicate with a central coordinator (server)). At each communication round $t$, the server sends the current global model to the clients, which in turn train the model on their local data, then send the model back to the server, which updates the global model with the average of the received models. More in detail, the Federated Learning problem is defined as:
%
\begin{align}
    % \*w_f^* =& \mathrm{argmin}_{\*w_f} \sum_{i=1}^{|\mathcal{V}|} p_i \frac{1}{|\mathcal{D}_i|}\sum_{j=1}^{|\mathcal{D}_i|}\ell(h(x_j;\*w_f),y_j)
    \*w_f =& \mathrm{argmin}_{\*w} \sum_{i=1}^{|\mathcal{V}|} p_i \underbrace{\frac{1}{|\mathcal{D}_i|}\sum_{k=1}^{|\mathcal{D}_i|}\ell\left(h\left(\*x_k;\*w\right),y_k\right)} \label{eq:fedlearn} \\
    & \phantom{============} F_i(\cdot) \nonumber{} 
\end{align}
%
where $h(\cdot; \*w)$ denotes the global model and $p_i$ is the relative weight of client $i$ and $\ell$ is the target loss function. Typically~\cite{wang_field_2021}, $p_i$ is set to $\frac{|\mathcal{D}_i|}{\sum_{\forall i \in \mathcal{V}}|\mathcal{D}_i|}$ (which reduces to $\frac{1}{|\mathcal{V}|}$ when local datasets have the same size), effectively weighting clients based on the amount of training data they have. The above global optimization problem is solved by FedAvg in a decentralized way by letting client devices, at each communication round $t$, perform a certain number of updates to minimize $F_i(\cdot)$ in \autoref{eq:fedlearn}. The local parameters' set $\*w_i^t = \textrm{argmin}_{\*w} F_i(\*w)$ resulting from the local optimization (e.g. using SGD) at communication round $t$ on node $i$ is then sent to the parameter server, which combines the local models as $\*w_f^t = \sum_{i=1}^{|\mathcal{V}|} p_i \*w_i^t$ to obtain $\*w_f^t$. Under common conditions, $\*w_f^t \sim \*w_f$ for $t$ sufficiently long~\cite{li_convergence_2020}\footnote{Note, though, that when data are non-IID and the learning rate $\eta$ of SGD is fixed, $\*w_f^t$ will be at least $\Omega(\eta (E-1))$ away from the optimal $\*w_f$, despite convergence. $E$ is the number of epochs for SGD.}. In the most general version of FedAvg, not all clients are involved in the training at each communication round (saving on per-device communications). 
% In that case, the aggregation function at the orchestrator becomes $\*w_f^t = \frac{\sum_{i=1}^{|\mathcal{S}^t|} p_i \*w_i^t}{\sum_{i=1}^{|\mathcal{S}^t|} p_i}$, where $\mathcal{S}^t$ denotes the set of clients selected to participate at communication round~$t$.

\noindent{}\emph{Communication overhead}: The nodes send their models to the central server at each communication round.

\noindent {\bf{Learning in isolation:}} 
% There is no central server (neither for the training nor for the aggregation, like in FedAvg).
The client devices train their local models $h(\cdot\; ; \*w_i)$ on their local data by minimizing a target loss function $\ell$ as follows:
%
\begin{equation}
\*w_i^* = \mathrm{argmin}_{\*w_i} \sum_{k = 1}^{|\mathcal{D}_i |} \ell(h(\*x_k;\*w_i), y_k)
\label{eq:isolation}
\end{equation}
%
with $(\*x_k, y_k) \in \mathcal{D}_i$.

\noindent{}\emph{Communication overhead}: nodes send nothing over the network.

\subsection{Decentralization baselines}
\label{sec:baselines_dec}

The general learning problem for fully decentralized settings, i.e., with no central server acting as the learning orchestrator, is the same as in Federated Learning (\autoref{eq:fedlearn}). However, this general learning problem cannot be solved anymore by relying on a special node that runs the aggregation and sends back the resulting model to the nodes in the network. In fact, while the FL orchestrator is connected to $|\mathcal{V}|$ nodes (effectively mapping the FL network topology to a star graph with the orchestrator at the center), each node $i$ in DFL is only connected to its neighbors (whose set we denote with $\mathcal{N}_i$). 
% Thus, repeated random sampling in $|\mathcal{V}|$ by the orchestrator guarantees that all nodes are picked on average with the same frequency, hence all local models will be fairly represented in the global model. Vice versa, whatever nodes in DFL takes care of the aggregation can only aggregate the model coming from $\mathcal{N}(i)$.

More in detail, at time $t=0$ the node $i$ trains the model $h(\cdot\; ; \*w_i^{(t)})$ on its data $D_i$ by minimizing a target loss function as in \autoref{eq:isolation}.
% More in detail, at time 0, the model $h(\cdot\; ; \*w_i)$ is, as usual, trained on local data, by minimizing a target loss function: $\*w_i^* = \mathrm{argmin}_{\*w_i} \sum_{k = 1}^{|\mathcal{D}_i |} \ell_i(h(\*x_k;\*w_i), y_k)$. Note that, at least in principle, each node can define its own local loss function for training the local model.
Then, the model $\*w_i^{(0)}$ is sent to all the neighbors in~$\mathcal{N}_i$. 
We assume that nodes entertain a certain number of \emph{communication rounds} $R$, exchanging and combining local models. At each communication round, a given node $i$ receives the local models from its neighbors in the graph, and aggregates them with its local model. The aggregation can be represented as follows:
%
\begin{equation}
    h(\cdot; \*w_i^{(t)}) \leftarrow \bigoplus_{j \in \mathcal{N}_i} h(\cdot; \*w_j^{(t-1)})
\end{equation}

Different decentralised aggregation functions will define the operator $\oplus$ differently. In the following of this section, we present the benchmark policies we will compare against.

\noindent {\bf{DecAvg:}}  In the simplest case (hereafter, DecAvg), at each step $t$, the local model of the given node and the local models from the node's neighbors are averaged FedAvg-style, as specified in the following:
%
\begin{equation}
    \*w_i^{(t)} \leftarrow \frac{\sum_{j \in \mathcal{N}(i)} \omega_{ij} p_{ij} \*w_j^{(t-1)}}{\sum_{j \in \mathcal{N}(i)} \omega_{ij}},
    \label{eq:decavg}
\end{equation}
%
% where $\omega_{ij}$ are the social weights introduced in Sec.~\ref{sec:preliminaries}, 
where $p_{ij}$ is equal to $\frac{|\mathcal{D}_j|}{\sum_{j \in \mathcal{N}_i} | \mathcal{D}_j|}$ (and captures the relative weight of the local dataset of node $j$ in the neighborhood of node $i$, similarly to parameter $p_i$ in federated learning's~\autoref{eq:fedlearn} but restricted to the local neighborhood of node $i$, since everything is decentralized). 

This strategy is the natural extension of FedAvg (the most well-known FL approach~\cite{mcmahan_communication-efficient_2017}) to a decentralized setting: the aggregation is performed not by the central controller (as in federated settings) but by each node, whereby each node averages the model received from a given neighbor based on the strength of the social link connecting them.

In this work, we consider two flavors for DevAvg, described below.

\noindent {\bf{DecAvg with initial coordination:}} We assume that nodes are able to coordinate initially to start learning from a \emph{common model}, i.e., $\*w_i^{(0)} = \*w_j^{(0)}, \forall i,j \in \mathcal{V}$.  This is not generally feasible in realistic settings (unless the network is very small and stable). However, it still provides a good benchmark for what decentralized learning can achieve under ideal conditions.

    \noindent{}\emph{Communication overhead}: nodes send their models to their neighbors in the graph and they have to run a coordination algorithm to exchange the initial model parameters from which everybody starts at time zero.

\noindent {\bf{DecAvg w/o coordination:}} We assume that nodes are \emph{not} able to coordinate initially to start learning from a common model, i.e., defining the NN topology but not the initialization of the parameters all over the network. Thus, $\*w_i^{(0)} \neq \*w_j^{(0)}, \forall i,j \in \mathcal{V}$. This assumption is much more realistic in practical settings but introduces novel challenges that we illustrate in Section~\ref{sec:motivating_example}.

\noindent{}\emph{Communication overhead}: nodes send their models to their neighbors in the graph.

In all cases, once the aggregation of models is performed, the local model is trained again on the local data. % (in this paper, we use learning rate $\eta$ and momentum $\mu$).

%================================================================================
\subsection{Motivating example}
\label{sec:motivating_example}

[dyadic/triadic + very simple strategies]

[integrate]
Despite being a very popular approach in a federated learning setting, DecAvg is expected to suffer in a decentralized environment from the lack of central coordination. In standard FedAvg, the server sends a common initial model to all nodes, which then starts the learning with common parameters. Without the common initialization, local models are expected to associate different features with different neurons (due to the permutation invariance of the hidden layers of neural networks). When this happens, coordinate-wise averaging can be detrimental (because nodes are averaging weights that do not match the corresponding learned features). However, the lack of a common initialization can only be solved by either forcing the nodes to coordinate in a decentralized way before the learning phase or exploiting strategies that do not require coordination. We believe that an initial coordination round is not suitable for dynamic decentralized scenarios (percolating the common initialization across the network might be time-consuming, the nodes of the networks may come and go, etc.). For the second approach, we discuss below some possible solutions. 

%==========================================================================
\section{Our contribution}
\label{sec:contribution}

The results in Section~\ref{sec:motivating_example} have shown the limits of na\"ive averaging in a fully decentralized scenario. Simple coordinate-wise averaging can be detrimental in a decentralized scenario because nodes are averaging weights that do not match the corresponding learned features. However, the lack of a common initialization can only be solved by either forcing the nodes to coordinate in a decentralized way before the learning phase or exploiting strategies that do not require coordination. We believe that an initial coordination round is not suitable for dynamic decentralized scenarios (percolating the common initialization across the network might be time-consuming, the nodes of the networks may come and go, etc.).

For the second approach, our proposal for tackling these challenges is based on two key ideas, discussed below. Nodes collaborating in a decentralized learning task perform three steps at each communication round: they aggregate the models they have received from their neighbors at the previous round into their local model, then retrain the updated aggregate model on the local data, and finally send the aggregate model to their neighbors. The strategies we propose affect the aggregation phase and the retraining phase. With the DecDiff aggregation that we propose, we aim to mitigate the issues coming from the lack of coordination in fully decentralized settings. With the virtual teacher mechanism that we leverage for the retraining, we aim to boost the knowledge extraction process from the local dataset without impacting either the communication or the computational overhead. 

\subsection{Aggregation with DecDiff}
\label{sec:decdiff}

The limitations of na\"ive averaging are mainly because the aggregation blindly moves toward the average of the neighbourhood model without first assessing whether this movement is going to be disruptive or not. To mitigate this problem, we propose to update the local model in the direction of the neighborhood-averaged model (like we did in DecAvg) but the shift toward the average should be less intense when the average model is distant (in $L_2$ norm) from the local one. In practice, in the initial communication rounds, when nodes are expected to be farthest, the local model makes small steps toward the average model. With these small steps, the intense initial disruption observed in Section~\ref{sec:motivating_example} will be avoided. We name this aggregation strategy DecDiff because it effectively factors in the model differences when performing the aggregation.

\noindent {\bf{DecDiff:}}  At each step $t$, the local model is updated according to the following update rule:
%
\begin{equation}
\*w_i^{(t)} = \*w_i^{(t-1)} - \frac{\bar{\*w}^{(t)} - \*w_i^{(t-1)}}{|| \bar{\*w}^{(t)} - \*w_i^{(t-1)} ||_2 + \*1},
\label{eq:decdiffupadte}
\end{equation}
%
where the average model $\bar{\*w}^{(t-1)}$ equal to $\*w_i^{(t)}$ in Equation~\ref{eq:decavg}.

\noindent{}\emph{Communication overhead}: nodes exchange their models with their neighbors at each time step.

\subsection{Virtual teacher}
\label{sec:virtual_teacher}

While DecDiff affects the aggregation phase of decentralized learning, in the following we discuss how to boost the training phase without generating additional communication costs. In a situation where nodes only see a small fraction of the whole training dataset, it is important to extract as much knowledge as possible from the data one has. Techniques based on knowledge distillation (KD)~\cite{hinton_distilling_2015} are known to do so. Briefly, in KD a (typically small) student deep neural network is trained to mimic the outputs of a bigger and well-trained one by minimizing the Kullback-Leibler divergence (KL) between the outputs of the two. Such a system is meant for centralized settings where both models can access the training data. Although there are some attempts to apply KD in decentralized settings, these works are based on the assumption that a teacher node has enough information to teach a student node how to answer a query correctly. However, in fully decentralized settings the presence of teacher nodes cannot be guaranteed. Conversely, we  assume that all the nodes hold only very partial information (since local datasets are non-IID) which might make their models strong only on some portion of data and very weak on other data. Summarizing, we assume that all the nodes' models are locally weak from the Teacher-Student (TS) paradigm point of view. 
However, according to \cite{yuan_revisiting_2020}, not only is it still possible to extract knowledge from poorly trained models through knowledge distillation, but in such a case, we can also overcome the need for a real teacher and use a virtual one implemented as soft labels (considering a classification problem). Specifically, each node defines a soft-labelling scheme for the local data and uses it to train the local model under the KD paradigm. So, rather than relying on a trained model, we can simply ``emulate'' a teacher. 
%
% Specifically, here we employ a \emph{virtual teacher} mechanism, inspired by~\cite{yuan_revisiting_2020}. 
% By definition, a teacher is a model with strong classification accuracy with respect to the student model. So, rather than relying on a trained model, we can simply ``emulate'' a teacher. 
To this aim, we set:
%
\begin{equation}
    p_t(y) =    \begin{cases}
                a & y=c\\
                (1-a)/(|\mathcal{L}|-1) & y \neq c
                \end{cases}
    \label{eq:vt}
\end{equation}
%
where $c$ is the correct label, and $a$ is the probability yielded for data belonging to that class. For a good teacher, it is reasonable to assume $a \geq 0.9$. The excess to 1 is equally spread among all other labels. Thus, during the training phase, we minimize:
%
% \begin{multline}
%     \mathrm{argmin}_{\*w} \sum_{j \in \mathcal{D}_i} (1-\alpha) \ell\left(y_j, h_i(\*x_j; \*w)\right) + \\
%     \alpha \ell_{KL}\left(p_i\left(\*x_j; \*w\right),p_{t}(l_j)\right),
%     \label{eq:decvt}
% \end{multline}
\begin{equation}
    \mathrm{argmin}_{\*w} \sum_{j \in \mathcal{D}_i} \ell_{KL}\left(p_i\left(\*x_j; \*w_i^{(t)}\right),p_{t}(y_j)\right),
    \label{eq:decvt}
\end{equation}
%
where $p_i\left(\*x_j; \*w_i^{(t)}\right)$ are the soft label probabilities extracted from $h_i(\*x_j; \*w_i^{(t)})$ and $p_{t}(l_j)$ are those returned from the virtual teacher model in Equation~\ref{eq:vt}.

\subsection{Proposed Algorithm}
The resulting algorithm is described in \autoref{alg:ddvt}. 
All the $K$ nodes in the system start by initialising the local model independently such that given nodes $i,j$, $\*w_i \neq \*w_j, \forall i,j\in K$ with $i\neq j$ and deciding the parameter $a$ for creating the local soft labels. This, combined with the non-iid data distribution  across them impose an additional level of heterogeneity. The local training is performed according to the standard procedure. Each nodes $k$ trains the local model for a number of epochs $E$ (which is not necessarily the same at all nodes) minimizing Eq.\ref{eq:decvt} (lines 3-8). In this paper we use SGD with momentum but the procedure holds for any optimization algorithm. Once the local training is complete, a node $k$ sends its local model the other nodes in its neighbourhood ($\mathcal{N}_k$) and receives the models sent by them (lines 11-12). Note that we do not impose any kind of synchronisation in this phase, thus at each communication round, a node might receive model from all or just a fraction of its neighbours. 
The set of models collected from the neighbourhood $\{w_n\}_{n\in\mathcal{N}_k}$ are used to compute the local average model $\bar{\*w}_k$ using a simple weighted average
\begin{equation}
    \bar{\*w}_k = \sum_{n\in\mathcal{N}_k} \rho_{k,n}\*w_n
    \label{eq:loc_avg}
\end{equation}
where the weighting parameter $\rho_{k,n}=\frac{|\mathcal{D}_n|}{\sum_{n\in\mathcal{N}_k} |\mathcal{D}_n|}$ is the portion of data that each node in the neighbourhood has (line 13). This weighting parameter is similar to the one initially proposed in \cite{mcmahan_communication-efficient_2017}, apart from the fact that it does not include the node $k$. In this way we build a reference average model that node $k$ is use \emph{as a driver} for performing the aggregation step (line 14). 
The nodes in the system perform the DecDiff+VT algorithm for number R of communication rounds. 
\begin{algorithm}
\caption{DecDiff+VT Algorithm}\label{alg:ddvt}
\begin{algorithmic}[1]
% \Require $n \geq 0$
% \Ensure $y = x^n$
% \State $y \gets 1$
% \State $X \gets x$
% \State $N \gets n$
% \While{$N \neq 0$}
% \If{$N$ is even}
%     \State $X \gets X \times X$
%     \State $N \gets \frac{N}{2}$  \Comment{This is a comment}
% \ElsIf{$N$ is odd}
%     \State $y \gets y \times X$
%     \State $N \gets N - 1$
% \EndIf
% \EndWhile
\State All $K$ nodes initialise the local model $\*w_k$ at random. 
\ForAll{$r=0\dots R$ all nodes $k\in K$}
\For{e=0,\dots,E}\Comment{Local training}
\For{b=0,\dots,E/bs}
\State Sample the $b$-th mini-batch $\boldsymbol\xi_b=(\*X_b,\*Y_b)$
\State Obtain soft labels $\tilde{\*Y}_b$ as in Eq.(\ref{eq:vt}) \Comment{output: probability vector}
\State Compute loss as in Eq.(\ref{eq:decvt})
\State Update model $w_b = \mathrm{SGD}(\eta,\mu)$
\EndFor
\EndFor
\State SendLocalModel($\*w_r,\mathcal{N}_k$)
\State Receive models from neighbours $\{\*w_n\}_{n\in\mathcal{N}_k}$
\State Compute local average model $\bar{\*w}_k = \sum_{n\in\mathcal{N}_k} \rho_k\*w_n$
\State Update local model as in Eq.(\ref{eq:decdiffupadte})
\EndFor
% \EndFor
\end{algorithmic}
\end{algorithm}

% [OLD TEXT BELOW]

% \paragraph{Decentralized Teacher-Student [DecTS]} This strategy exploits a teacher-student approach, whereby, for each label $l$, a node from the neighborhood of node $i$ is elected teacher, and node $i$ tries to imitate the output of the teachers instead of combining models via averaging. Let us denote with $\mathcal{L}$ the set of all labels for data in $\mathcal{D}$. Then, after collecting the models from its neighborhood, node $i$ minimizes the following loss:
% %
% \begin{equation}
%     %\mathrm{argmin}_{\*w} \sum_{j \in \mathcal{D}_i} \ \ell\left(y_j, f_i(\*x_j; \*w)\right) +  \ell_{KL}\left(p\left(z_i^{j}\right),p\left(z_{t(j)}^{j}\right) \right)
%     \mathrm{argmin}_{\*w} \sum_{j \in \mathcal{D}_i} (1-\alpha) \ell\left(y_j, f_i(\*x_j; \*w)\right) +  \alpha \ell_{KL}\left(p_i\left(\*x_j; \*w\right),p_{t(l_j)}\left(\*x_j; \*w)\right) \right)
%     \label{eq:dects}
% \end{equation}
% %
% where we denote with $\ell_{KL}$ the Kullback-Leibler distance, with $p_i$ the softmax output of node $i$, and with $p_{t(j)}$ the softmax output of the teacher of the class label of $x_j$. 

% \emph{Communication overhead}: nodes exchange their models with their neighbors at each time step [@Lorenzo: can we save resources by simply exchanging the current accuracy + the probability vectors (averaged on the data local to the teacher)?].

% \paragraph{Decentralized Virtual Teacher [DecVT]} Inspired by~\cite{yuan_revisiting_2020}, here we test the effectiveness of a virtual teacher. By definition, a teacher is a model with strong classification accuracy with respect to the student model. So, rather than relying on a trained model, like in DecTS, we can simply ``emulate'' a teacher. To this aim, we set:
% %
% \begin{equation}
%     p_t(k) =    \begin{cases}
%                 a & k=c\\
%                 (1-a)/(|\mathcal{L}|-1) & k \neq c
%                 \end{cases}
% \end{equation}
% %
% where $c$ is the correct label and $a$ is the probability yielded for data belonging to that class. For a good teacher, it is reasonable to assume $a \geq 0.9$. The excess to 1 is equally spread among all other labels. Thus, Equation~\ref{eq:dects} becomes:
% %
% \begin{equation}
%     \mathrm{argmin}_{\*w} \sum_{j \in \mathcal{D}_i} (1-\alpha) \ell\left(y_j, f_i(\*x_j; \*w)\right) +  \alpha \ell_{KL}\left(p_i\left(\*x_j; \*w\right),p_{t}(l_j)\right)
%     \label{eq:decvt}
% \end{equation}

% \emph{Communication overhead}: nodes do not exchange anything.

%==========================================================================
\section{Experimental settings}
\label{sec:settings}

In order to evaluate the learning strategy proposed in Section~\ref{sec:contribution}, we focus on a fully decentralized collaborative image classification task. For the experiments, we use a custom Python simulator (\textsc{SaiSim}) that integrates graph generation (via the \texttt{networkx} library), deep learning functionalities (via the \texttt{PyTorch} library) and offers novel routines to support fully decentralized learning\footnote{A link to the simulator code will be released in the camera ready of the paper, if accepted.}. We perform four replicas for each scenario described below, reporting $95\%$ confidence intervals when relevant.


\subsubsection{Social network topology}
\label{sec:topology}

We consider an Erd\H{o}s–R\'enyi $G(n, p)$ graph with 50 nodes and edge creation probability set to $0.2$, which is well above the critical value $0.078$ (computed from $\frac{\ln(50)}{50}$ \cite{erdHos1960evolution}). This means that the network is almost surely connected. The latter property is important to avoid degenerate situations where nodes exist that cannot communicate with anyone else. Disconnected nodes are forced to operate in isolation, hence they would not be suitable for assessing the properties of decentralized learning. We do believe that investigating the impact of network connectivity on the performance and robustness of decentralized learning is a critical research problem to be tackled, but it does not fit within the scope of this paper and we leave it as future work. The specific instance of the Erd\H{o}s–R\'enyi graph used for our simulation is shown in~\autoref{fig:graph}.

\begin{figure}[t]
\centering
\includegraphics[scale=0.8]{figures/graph.pdf}
\caption{The Erd\H{o}s–R\'enyi graph we used for simulations. The vertex size and colour (from green to white) are proportional to the node degree.}
\label{fig:graph}
\end{figure}


\subsubsection{Datasets}
\label{sec:datasets}

We consider the following different datasets.

\noindent MNIST: This dataset is a collection of handwritten digits. It consists of 60,000 training examples and 10,000 test examples. Each example is a grayscale image of size 28x28 pixels, representing a single digit from 0 to 9. The digits are handwritten by various individuals, making the dataset diverse in terms of writing styles and quality.

\noindent FASHION-MNIST: This dataset contains 10 different types of fashion item images. The number of training/test examples is the same as for MNIST, as well as the grayscale image pixel size.

\noindent EMNIST: This dataset is an extension of the original MNIST dataset that includes both handwritten digits and handwritten letters. Here we consider only the split EMNIST Letters, which focuses exclusively on uppercase letters. It consists of 26 classes, with 20,800 training examples and 3,280 test examples.

\subsubsection{Data allocation}
\label{sec:data_allocation}

In order to reproduce a realistic scenario, data items from the training set are distributed in a non-IID way across nodes. Specifically, class images are assigned to nodes according to a Zipf distribution with exponent $\alpha_{zipf}=1.26$, to guarantee sufficiently skewed distributions, as explained next. For each class, we draw 50 Zipf samples, whose values correspond (approximately, see the limitation of boundary effects below) to the number of images for that class assigned to the node. 
This approach yields a very skewed data distribution, where one node has the majority of images for that class. In order to avoid boundary effects caused by nodes with zero images for a certain class, we guarantee that all nodes see at least some images for each class, however few. An example allocation for the EMNIST dataset is shown in \autoref{fig:data_distribution}. Such skewed data distribution implies that no node alone can perform well on the test set where all classes are present. Thus, collaboration among nodes becomes crucial.

\begin{figure}[t]
\centering
\includegraphics[width=.95\columnwidth]{figures/data_distribution_circles-emnist.pdf}
\caption{Example of data distribution over nodes for EMNIST.}
\label{fig:data_distribution}
\end{figure}

Due to the potentially disruptive effect on the learning process of skewed data distribution across nodes, it is important to capture quantitatively how skewed the data allocation is in each simulation run. To this aim, we leverage the Gini Index (GI), which is a standard inequality metric. The Gini Index ranges from 0 (perfect equality) to 1 (absolute inequality). Our goal is to tackle a fairly heterogeneous data distribution, thus we work in the range $[0.7, 0.85]$. For all plots concerning single simulation runs, we report the Gini index associated with the instance of data heterogeneity in that run. 
\ifextremehetero
To complement this analysis, we consider an extremely skewed distribution ($GI > 0.9$) in Section~\ref{sec:extreme_heterogeneity}.
\fi

\subsubsection{Local model architecture}
\label{sec:local_model_architecture}

\begin{table}
\centering
\caption{NN models architectures used in this paper}
\label{tab:nn_topology}
\begin{tabular}{llp{.1\textwidth}ll}
\toprule
\textbf{Dataset} & \textbf{Model} & \textbf{Structure} & \textbf{Activation} & \textbf{Kernel size} \\
\midrule
MNIST & MLP & FC:512,256,128  & ReLU & - \\
Fashion & CNN & Conv2d:32,64\newline FC:9216,128 & ReLU & 3$\times$3 \\
EMNIST & CNN & Conv2d:32,64\newline MaxPool(2)\newline Dropout(.25) \newline FC:9216,128\newline Dropout(.5)\newline FC:128 & ReLU & 3$\times$3 \\
\bottomrule
\end{tabular}
\end{table}

We use different local model architectures for the different datasets, as reported in \autoref{tab:nn_topology} As optimizer we use SGD with the following configurations. For MNIST  we set the learning rate $\eta = 0.001$ and the momentum $\mu = 0.5$. For FASHION-MNIST and EMNIST we set the learning rate $\eta = 0.001$ and the momentum $\mu = 0.9$.

For all strategies except Centralized and FedAvg, the model parameters are drawn at random locally at each node. This implies that nodes start with different model initialization, as is to be expected in realistic decentralized settings.

\subsubsection{Benchmarks}
\label{sec:benchmarks}

We compare decentralized learning against the following benchmarks.

% \item[DecTS-Oracle] The upper bound to a teacher-based learning is when the teacher is as good as they get, i.e., the teacher model is exactly the centralized model obtained with \emph{Central learning}. This baseline is not meaningful in practice, but it provides an estimate of the potential of TS learning: if DecTS-Oracle does not beat another target strategy, there is no designing an alternative teacher that can be that [@Lorenzo: actually, this might not be true? Some noise could prove useful?]. 

\noindent {\bf{CFA:}} Consensus-based Federated Averaging has been proposed by~\cite{savazzi_federated_2020}. Aggregation is performed as follows:
%
\begin{equation}
    \*w_i^{(t)} = \*w_i^{(t-1)} + \epsilon \sum_{j \in \mathcal{N}_i} p_{ij} \left( \*w_j^{(t-1)} - \*w_i^{(t-1)} \right),
    \label{eq:cfa}
\end{equation}
%
with $p_{ij} = \frac{|\mathcal{D}_j|}{\sum_{k \in \mathcal{N}_i} |\mathcal{D}_i|}$ and $\epsilon \in \left(0, \frac{1}{\Delta}\right)$, with $\Delta=|\mathcal{N}(i)|$. As in the follow-up work~\cite{savazzi_framework_2021}, we set $\epsilon = \frac{1}{\Delta}$.
% but in~\cite{savazzi_federated_2020} they seem to assume $\Delta = 1$ (with $\epsilon_t$ set to 0.5 or 1)
% When $\epsilon_t = 1$, CFA is equivalent to DecAvg, while when $\epsilon_t = |\mathcal{N}_i|$, the local model weighs much more than the others (i.e., $\frac{1}{\mathcal{N}_i}\left[(\mathcal{N}_i-1)\*w_i + \sum_{k \in \mathcal{N}_i \bigcup \{i\}} \alpha_{i,k} \*w_k\right]$).

\noindent {\bf{CFA-GE:}} It has been proposed in~\cite{savazzi_federated_2020}, as a variation of CFA, where \emph{both} models and local gradients are exchanged at each communication round. Specifically, after the aggregation (performed as in~\autoref{eq:cfa}), node $i$ sends the model parameters $\*w_i^{(t)}$ to its neighbors and asks them to use the model to compute the gradients on the neighbors' local data. Once computed, the neighbors send the gradient back to node $i$, which then updates model  $\*w_i^{(t)}$ with the received gradients. In our implementation, we use the speed-up implementation proposed in~\cite{savazzi_federated_2020}.
%
This model is expected to perform generally well due to the exploitation of gradients trained on neighbors' data. However, it has a high communication and computation overhead since nodes are expected to exchange their gradients as well as their models with their neighbors and to train their neighbors' models on local data. While this could be infeasible in practice on user devices, it is still interesting to consider this approach as one of the benchmarks. 

\section{Results}
\label{sec:results}
\subsection{Performance comparison with non-IID data}
\label{sec:accuracy}
\begin{table*}[ht]
\centering
\caption{Average accuracy on MNIST, Fashion-MNIST, EMNIST}
\label{tab:avg_acc_all}
\begin{tabular}{@{}llllllll@{}}
\toprule
& & \multicolumn{2}{c}{MNIST} & \multicolumn{2}{c}{Fashion-MNIST} & \multicolumn{2}{c}{EMNIST} \\
& Method & \bf{Avg accuracy} & \bf{CI half interval} & \bf{Avg accuracy} & \bf{CI half interval} & \bf{Avg accuracy} & \bf{CI half interval}\\ 
\midrule
\multirow{2}{*}{\par{Standalone baselines}}&Centralised & 0.9824 & 0.00000 & 0.9181 & 0.00000 & 0.9027 & 0.00000 \\ 
& ISOL & 0.6473 & 0.09001 & 0.7594 & 0.03919 & 0.4654 & 0.08640 \\ 
\midrule
Distributed baseline & FED & 0.9410 & 0.01564 & 0.8939 & 0.00335 & 0.8344 & 0.02111 \\ 
\midrule
\multirow{3}{*}{Decentralised SOTA}& DecHetero & 0.9071 & 0.02487 & 0.8837 & 0.00288 & 0.8301 & 0.02782 \\ 
& CFA & 0.8975 & 0.03063 & 0.8568 & 0.00477 & 0.7807 & 0.03453 \\ 
& CFA-GE & 0.9460 & 0.00476 & 0.8564 & 0.01298 & 0.8607 & 0.00920 \\ 
\midrule
\multirow{2}{*}{Decentralised Proposal}& DecDiff & 0.9373 & 0.01526 & 0.8838 & 0.00459 & 0.8214 & 0.02575 \\ 
& DecDiff+VT & \bf{0.9530} & 0.01536 & \textbf{0.8904} & 0.00427 & \bf{0.8653} & 0.01276 \\ 
\bottomrule
\end{tabular}
\end{table*}
Whatever the specific decentralised learning strategy, the goal of decentralised learning is to approach the performance of its centralised counterpart. More realistically, given that the latter is an ambitious goal for decentralised learning, we strive to perform similarly a centrally controlled approach as federated learning. Therefore, we compare the results of our proposed solution against three different types of benchmarks: (i) the standalone baselines where no cooperation between devices is involved, (ii) the standard federated learning framework where a parameter server coordinates the learning process and (iii) the decentralised framework where there is cooperation but no coordination between devices. In the following, we will refer to \autoref{tab:avg_acc_all}. 

The performance of the standalone approaches, i.e., Centralised and Isolation, constitutes the two extremes of the obtainable performance range. Given a DNN model and a dataset, the former represents the upper bound that all the distributed and decentralised learning approaches should achieve. In contrast, the latter represents the lower bound we would obtain without cooperation between devices. The gap between the two expresses the maximum gain from using a decentralised learning scheme. In our settings and depending on the specific learning configuration, the expected average gains are 34\% (MNIST), 15\% (Fashion-MNIST) and 45\% (EMNIST). Finally, the Federated Learning (FL) performance stands between Centralised and Isolation. It represents a second reference benchmark since the operating conditions are more favourable w.r.t. a fully decentralised system, i.e., the parameter server is a single aggregation point, and all the clients train the same global model. Our solution DecDiff+VT achieves comparable or even better performance than FL w\ FedAvg across all the datasets. Precisely, on Fashion-MNIST, the final average accuracy is statistically equivalent to FL, while on MNIST and EMNIST nodes, predictions are 1.20\% and 3.09\% more accurate.

These results suggest that our solution can overcome difficulties induced by two sources of heterogeneity: data and models' initialisation. This is also confirmed by looking at the performance of the decentralised benchmarks. DecHetero represents the equivalent of FL in decentralised settings with a lack of coordination between the devices regarding the models' initialisation. Comparing its performance with standard FL, we observe that the additional source of heterogeneity is particularly detrimental and causes an additional degradation in the overall performance, i.e., depending on the specific dataset, the devices can lose up to 3.39\% accuracy (MNIST). The reason for such degradation is rooted in the averaging mechanism that, when applied to models initialised differently and trained on non-IID data, destroys the information previously learnt by the models.
Nonetheless, the averaging also acts as a (partial) synchronisation event, after which the nodes find a partial agreement w.r.t. their neighbourhood. During the following updates, the divergence between models gets smaller and smaller, and the primary source of heterogeneity is due to the relative difference of their local datasets, from which FedAvg can recover, as suggested by the closeness of the final performance to the FL ones. 
Our solution does not suffer such shortcomings, although we still use the neighbourhood-wise average model to drive the devices' local model updates. Our difference-based update combined with the virtual teacher-based local training makes the models' updates less susceptible to both sources of heterogeneity, i.e., models initialisation and non-iid-ness, by smoothing the models' parameters convergence in the neighbourhood and thus making the whole process less disruptive through time.
Let us compare the performance with the decentralised direct competitors CFA and CFA-GE. The aggregation step of CFA is based on the weighted difference between the local and the neighbourhood models. The update is scaled proportionally to the size of the neighbourhood. In our case, the update is based on the difference between the local and neighbourhood-wide aggregate models. Such a slight variation significantly impacts the robustness of our approach to heterogeneity. Table \ref{tab:avg_acc_all} shows that Decdiff+VT outperforms CFA on all the datasets, improving the performance by 5.55\% (MNIST), 3.33\% (Fashion-MNIST), 8.46\% (EMNIST). CFA-GE aggregation step solves some of the weaknesses introduced by CFA by exploiting not only the information provided by the model parameters but also the gradients computed on the neighbourhood local data, as demonstrated by the average accuracy improvement reported in \autoref{tab:avg_acc_all}. It is worth noting that this improvement comes at an additional cost in terms of communication and computation, i.e., nodes exchange not only models but also gradients computed using previous versions of the neighbours' models, doubling the information transmitted in the system and increasing the computational effort by a factor that grows linearly with the size of the neighbourhood. Decdiff+VT show better or statistically equivalent performance than CFA-GE, without additional communication or computational effort. 
% <passare a dire che CFA é un meccanismo basato sulle differenze come il nostro ma che use un metodo di scaling differente che rende molto lento il travaso di informazione da un nodo all'altro. Problema risolto con CFA-GE ad un costo computazionale e di comunicazione maggiorato. Ciononostante il nostro approccio riesce a ottenere risultati migliori di entrambi senza costi aggiuntivi. DONE

% Vanno mostrati anche i valori di train e test loss. 

% poi bisogna passare alle velocità di convergenza.

% poi massiamo alla ablation analysis mostrando come impatta DecDiff e VT 

%  infine mostrare la matrice delle distanze in cui si vede che il nostro approccio portai i modelli a confergenza (o quasi). <qui non servono confronti secondo me> 


\subsection{Test loss analysis and characteristic time}

\begin{table}[t!]
\centering
\caption{Avergae characteristic time (in number of communication rounds) w.r.t. the accuracy of the centralised benchmark.}
\label{tab:conv_time}
\begin{tabular}{llrrrr}
  \toprule
Dataset & Method & 50\% & 80\% & 90\% & 95\% \\ 
  \midrule
\multirow{7}{*}{MNIST}& DecHetero & 97.400 & 235.600 & 583.250 & -  \\ 
  &CFA & 109.400 & 322.400 & 609.667 & - \\ 
  &CFA-GE & 102.800 & 173.400 & \bf{327.600} & 691.600 \\ 
  &DecDiff & \bf{52.800} & \bf{145.400} & 395.600 & 671.000 \\ 
  &DecDiff+VT & 55.200 & 161.000 & 360.000 & \bf{540.750} \\ 
  \cmidrule{2-6}
  &FED & 11.800 & 57.400 & 307.400 & 662.667 \\ 
  &ISOL & 262.200 & - & - & - \\ 
   \midrule
\multirow{7}{*}{Fashion}&DecHetero & \bf{3.200} & \bf{53.200} & 387.200 & - \\ 
  & CFA & 10.600 & 142.400 & - & - \\ 
  & CFA-GE & 10.200 & 118.400 & 693.600 & -\\ 
  & DecDiff & 6.800 & 54.000 & 319.800 & -\\ 
  &DecDiff+VT & 7.000 & 53.800 & \bf{313.600} & -\\ 
  \cmidrule{2-6}
  &FED & 1.200 & 25.000 & 216.000 & -\\ 
  &ISOL & 3.800 & - & - & -\\ 
   \midrule
\multirow{7}{*}{EMNIST}&DecHetero & 22.000 & \bf{91.000} & 370.500 & - \\ 
  &CFA & 62.800 & 418.000 & - & - \\ 
  &CFA-GE & 33.200 & 167.000 & 324.200 & 812.250 \\ 
  &DecDiff & 17.600 & 107.200 & 566.750 & - \\ 
  &DecDiff+VT & \bf{9.600} & 106.800 & \bf{138.400} & \bf{400.250} \\ 
  \cmidrule{2-6}
  &FED & 4.000 & 53.800 & 322.250 & - \\ 
  &ISOL & 28.000 & - & - & - \\ 
  \bottomrule
\end{tabular}
\end{table}

\autoref{tab:avg_acc_all} shows that our Decdiff+VT solution consistently outperforms the competitors in terms of accuracy. Let us now analyse how the learning evolves over the communications rounds. To this end, refer to \autoref{tab:conv_time} where we report the characteristic times w.r.t the accuracy of the centralised benchmark for all the considered methods, including FED and ISOL, even though they are not direct competitors. We highlight the minimum time for each relative accuracy, i.e., the fastest method that reaches a certain relative accuracy w.r.t. the centralised benchmark. Let us focus on the decentralised methods.
Our solution, DecDiff+VT, is the fastest on all the datasets. Precisely, on MNIST and EMNIST, only DecDiff+VT and CFA-GE consistently exceed the 95\% threshold, and the former is 1.28$\times$ and 2$\times$ faster than the latter, respectively. In Fashion-MNIST, although none of the considered solutions reach the 95\% threshold but only the 90\%, DecDiff+VT is 2.2$\times$ faster than CFA-GE. 

Interestingly, DecDiff and DecDiff+VT are generally faster than (MNIST and EMNIST) or comparable to (Fashion) competitors in embedding constructively the knowledge contained in the received models during the initial communication rounds. Moreover, DecDiff+VT shows the ability to constantly learn and improve even when the other competitors stop learning and start to overfit the local data. As shown in Figures \ref{fig:mnist_test},\ref{fig:fashion_test},\ref{fig:emnist_test}, it is clear that for CFA-GE and DecDiff-VT the test loss keeps its descent when one of the others start slowing down or even increasing. These two methods show very similar behaviour, which is impressive if we consider that DecDiff+VT does not exploit any of the additional information contained in the gradients received from the neighbourhood as in CFA-GE. Moreover, apart from the initial communication rounds, DecDiff+VT is generally faster than CFA-GE. 


% \begin{figure}[t]
% \centering
% \includegraphics[width=1.0\columnwidth]{figures/loss_over_commrounds_mean_test-mnist.pdf}
% \label{fig:mnist_test}
% \end{figure}
% \begin{figure}[t]
% \centering
% \includegraphics[width=1\columnwidth]{figures/loss_over_commrounds_mean_test-fashion.pdf}
% \label{fig:fashion_test}
% \end{figure}
% \begin{figure}[t]
% \centering
% \includegraphics[width=1\columnwidth]{figures/loss_over_commrounds_mean_test-emnist.pdf}
% \label{fig:emnist_test}
% \end{figure}

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=1.0\columnwidth]{figures/loss_over_commrounds_mean_test-mnist.pdf}
         \caption{}
         \label{fig:mnist_test}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=1\columnwidth]{figures/loss_over_commrounds_mean_test-fashion.pdf}
         \caption{}
         \label{fig:fashion_test}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=1\columnwidth]{figures/loss_over_commrounds_mean_test-emnist.pdf}
         \caption{}
         \label{fig:emnist_test}
     \end{subfigure}
        \caption{Test loss}
        \label{fig:three graphs}
\end{figure}

\subsection{Node-wise analysis}
Until now, we analysed the aggregate performance of all the nodes in the system, which reflects the system's global behaviour. In the following, we analyse the performance of the single nodes at the last communication round. Figure\ref{fig:pernode_acc} reports, for each methodology and each dataset, the accuracy achieved by each node in the system. The first interesting aspect to observe regards the dispersion of accuracy that the nodes achieve in isolation (ISOL), particularly evident in Fashion-MNIST and MNIST. The effect of cooperation is evident by looking at the accuracy distribution of the decentralised approaches. However, for some of them (i.e., DecHetero, CFA, DecDiff), the accuracy distribution still results rather dispersed, suggesting that, in highly heterogeneous settings, neither a naive application of the decentralised version of FedAvg nor some more sophisticated approaches (i.e., CFA, DecDiff) to make the nodes exploit all the knowledge contained in their local data. Differently, only DecDiff+VT and CFA-GE result in a more concentrated distribution of accuracy, highlighting in our solution the role of the Virtual Teacher, as it becomes evident in Figure\ref{fig:pernode_acc}-c. 

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=1.0\columnwidth]{figures/accuracy_over_commrounds_boxplot-mnist.pdf}
         \caption{}
         \label{fig:mnist_test}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=1\columnwidth]{figures/accuracy_over_commrounds_boxplot-fashion.pdf}
         \caption{}
         \label{fig:fashion_test}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=1\columnwidth]{figures/accuracy_over_commrounds_boxplot-emnist.pdf}
         \caption{}
         \label{fig:emnist_test}
     \end{subfigure}
        \caption{Node-wise accuracy at the last communication round.}
        \label{fig:pernode_acc}
\end{figure}

%=========================================================
\ifextremehetero
\subsection{Performance under extreme data heterogeneity}
\label{sec:extreme_hetero}

TBD

\fi

%=========================================================
\subsection{Communication efficiency}
\label{sec:communication_overhead}

%=========================================================
\subsection{Sensitivity analysis of $\beta$ parameter}
\label{sec:sensitivity}

%=========================================================

\section{Conclusion}
\label{sec:conclusion}
The conclusion goes here.

\appendix

% data distribution

% train loss
